Source-to-source optimizing transformations of Prolog programs based on abstract interpretation

Making a Prolog program more efficient by transforming its source code, without changing its operational semantics, is not an obvious task. It requires the user to have a clear understanding of how the Prolog compiler works, and in particular, of the effects of impure features like the cut. The way a Prolog code is written - e.g., the order of clauses, the order of literals in a clause, the use of cuts or negations - influences its efficiency. Furthermore, different optimization techniques may be redundant or conflicting when they are applied together, depending on the way a procedure is called - e.g., inserting cuts and enabling indexing. We present an optimiser, based on abstract interpretation, that automatically performs safe code transformations of Prolog procedures in the context of some class of input calls. The method is more effective if procedures are annotated with additional information about modes, types, sharing, number of solutions and the like. Thus the approach is similar to Mercury. It applies to any Prolog program, however.

==> biblio.tex <==

\begin{thebibliography}{10}

\bibitem{AitKaci91-WAM}
H. A\"{i}t-Kaci. {\em Warren's Abstract Machine: A Tutorial Reconstruction}. 1991. The MIT Press. London.

\bibitem{Apt97-Book}
K.R. Apt. {\em From Logic Programming to Prolog}. Prentice Hall, 1997.

\bibitem{Bruynooghe91-PracticalFramework}
Bruynooghe, M. 1991. {\em A practical framework for the abstract interpretation of logic programs.} J. Log. Program. 10, 2 (Jan. 1991), 91-124.

\bibitem{Cortesi00-Combination}
A.~Cortesi, B.~Le~Charlier, P.~Van~Hentenryck. {\em Combination of abstract domains for logic programming: open product and generic pattern construction}. Science of Computer Programming 38:27--71, Elsevier Science 2000.

\bibitem{Debray90-BanishingCut}
S. K. Debray and D. S. Warren. {\em Towards Banishing the Cut from Prolog.} IEEE Trans. Softw. Eng. 16, 3 (Mar. 1990), 335-349. 1990.

\bibitem{Deville90-Book}
Y. Deville. {\em Logic Programming:Systematic Program Development}. A. Wesley, 1990.

\bibitem{Gobert07-AFADL}
F. Gobert and B. Le Charlier. {\em A System to check Operational Properties of Logic Programs}. AFADL'07 conference. Namur. 2007.

\bibitem{Hermenegildo05-IntegratedProgramDebuggingVerificationOptimization}
M. Hermenegildo, G. Puebla, F. Bueno, P. L\'opez-Garc\'ia. {\em Integrated Program Debugging, Verification, and Optimization Using Abstract Interpretation (and The Ciao System Preprocessor).} Science of Computer Programming, Vol. 58, Num. 1-2, pages 115-140, Elsevier Science, October 2005.

\bibitem{GAIA}
B.~Le~Charlier and P.~Van~Hentenryck. {\em Experimental Evaluation of a Generic Abstract Interpretation Algorithm for Prolog}. {ACM Transactions on Programming Languages and Systems (TOPLAS)}, 16(1):35--101, January 1994.

\bibitem{LeCharlier99-Automatic}
B.~Le~Charlier, C.~Lecl\`ere, S.~Rossi, and A.~Cortesi. {\em Automated Verification of Prolog Programs.} JLP, 39:3--42, Elsevier Science 1999.

\bibitem{LeCharlier02-SequenceBased}
B.~Le~Charlier, S.~Rossi, and P.~Van~Hentenryck. {\em Sequence-Based Abstract Interpretation of Prolog}. {TPLP} 2(1): 25-84 (2002)

\bibitem{Somogyi96-Mercury}
{Z.Somogyi, F.Henderson, T.Conway.}$\!\!$
{\em The Execution Algorithm of Mercury, an Efficient Purely Declarative Logic Programming Language}.$\!\!\!$
{JLP}, 29(1--3):17--64, 1996.

\bibitem{SterlingShapiro94-ArtOfProlog}
L. Sterling and E. Shapiro. {\em The Art of Prolog, Advanced Programming Techniques}. Second Edition. The MIT Press. 1994. Cambridge, Massachusetts. London.

\bibitem{Warren83-WAM}
D. H. D. Warren. {\em An abstract Prolog instruction set}. Technical Note 309, SRI International, Menlo Park, CA, October 1983.

\bibitem{SwiProlog}
J. Wielemaker. {\em SWI-Prolog 5.6 Reference Manual.} University of Amsterdam. April 2006.
{\em http://www.swi-prolog.org}

\end{thebibliography}


==> table-append.tex <==


\begin{table}[h]
\begin{center}
\begin{tabular}{|l|r|r|r|r|r|}
\hline
\multicolumn{1}{|c|}{\bf Input} & \multicolumn{3}{c|}{\bf Execution Time (ms)} & \multicolumn{2}{c|}{\bf Local Stack (By)} \\
\cline{2-6}
\multicolumn{1}{|c|}{\bf list}  & \multicolumn{1}{c|}{\bf Multidirectional} & \multicolumn{2}{c|}{\bf Optimized} & \multicolumn{1}{c|}{\bf Multidirectional} & \multicolumn{1}{c|}{\bf Optimized}\\
%\cline{2-6}
\multicolumn{1}{|c|}{\bf size}  & \multicolumn{1}{c|}{\bf (ms)} & \multicolumn{1}{c|}{\bf (ms)} & \multicolumn{1}{c|}{\bf (sdup)} & \multicolumn{1}{c|}{\bf (By)} & \multicolumn{1}{c|}{\bf (By)} \\
\hline
100     &       &       &       &         &    \\
1000    &       &       &       &         &    \\
10000   &       &       &       &         &    \\
25000   &       &       &       &         &    \\
\hline
\end{tabular}
\end{center}
\caption{Execution of program {\tt append(L1,L2,L3)}, when {\tt L1} and {\tt L2} are ground lists, and {\tt L3} is a variable. The {\bf Input} column describes the list-length of {\tt L1}. The program has been tested on a 1.5~Ghz~Pentium; 1Gb~RAM; Linux~Suse; SWI-Prolog~v~5.4.6~\cite{SwiProlog}. The size to which the local stack is allowed to grow is 2048000 By.} \label{table-efface}
\end{table}


